ggViz: Accelerating Large-Scale Esports Game Analysis

While esports organizations are increasingly adopting practices of conventional sports teams, such as dedicated analysts and data-driven decision-making, video-based game review is still the primary mode of game analysis. In conventional sports, advances in data collection have introduced systems that allow for sketch-based querying of game situations. However, due to data limitations, as well as differences in the sport itself, esports has seen a dearth of such systems. In this paper, we leverage player tracking data for Counter-Strike: Global Offensive (CSGO) to develop ggViz, a visual analytics system that allows users to query a large esports data set through game state sketches to find similar game states. Users are guided to game states of interest using win probability charts and round icons, and can summarize collections of states through heatmaps. We motivate our design through interviews with esports experts to especially address the issue of game review. We demonstrate ggViz's utility through detailed case studies and expert interviews with coaches, managers, and analysts from professional esports teams.

==> 04_play_clustering_old.tex <==
\section{Play Clustering} \label{sec:play-clustering}

\subsection{Counter-Strike Description} \label{sec:csgo-description}
Counter-Strike: Global Offensive (CSGO) is a popular first-person shooter (FPS) video game where two teams of five players compete across a variety of objectives. A professional game takes place over one or more \textit{maps}, which are distinct virtual worlds. Most professional CSGO games are structured as a best of three maps. There is a pool of seven maps for competitive play, so to determine the three maps played in a game, each team participates in a picking and banning process before the game to determine which maps are played. On each map, teams are initially assigned a side, either the Terrorists (T) or the Counter-Terrorists (CT), and then play for 15 rounds as their assigned side. The two teams switch sides after 15 rounds. A team wins a map by winning 16 rounds.

Both the T and CT sides can win a round by completing a variety of objectives, such as eliminating all members of the opposing side, having the bomb explode or be defused, or running out of time. Both sides can win a round if they eliminate all members of the opposing side. The T side can win a round by planting and exploding a bomb at one of the two bombsites on a map, denoted A or B. At the start of each round, one T player is assigned the bomb. The bomb can only be planted at one of two bombsites. Once planted, the bomb explodes in 35 seconds, unless defused by the CT side. If the CT side successfully defuses the bomb, they win the round. If no win condition is met by the end of the round time (which is roughly two minutes), the CT side wins by default. Players start each round with 100 health points (HP) and are eliminated from a round when they reach 0 HP. Specifically, players lose HP when they are damaged -- typically from gunfire and grenades from the opposing side. Players buy equipment, such as guns, grenades (also called utility) and armor, at the beginning of a round, using virtual money earned from doing well in previous rounds. 

\subsection{CSGO Data} \label{sec:csgo-data}

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{imgs/csgo_data_pipeline_lato.pdf}
    \Description[CSGO data generation]{Esports are often structured in a client-server environment. We parse CSGO demo files, which record the game server updates.}
    \caption{Clients (players) provide input through keystrokes and mouse clicks, which changes their local game state. Clients then send these local game states to the game server, which reconciles the client states and sends a global game state back to all clients. While doing so, the server writes the global state to a demo file, which we then parse to generate a JSON containing spatiotemporal information about a match, including player events and trajectories.}
    \label{fig:demofile_generation}
\end{figure}

CSGO games take place in a client-server architecture. The clients (players) connect to a game server where they play their games. Client inputs, such as keyboard presses and mouse clicks, are recorded by the server and resolved across all clients every \textit{tick}. In competitive play, there are 128 ticks in a second, meaning a tick is roughly 8 milliseconds. Additionally, server side changes, such as round starts and ends, or bomb explosions, are also resolved across all clients. We show how these events are generated, and their parsed output, in Figure~\ref{fig:demofile_generation}.

A game can be recorded by the server through the use of a \textit{demo file} (\texttt{.dem}). The demo file contains a serialization of all client-server communications. When a demo file is recording, it writes data in tick bursts, which contain around eight ticks~\cite{bednarek2017data}. While a demo file can be recorded by a client, we focus solely on server-recorded demo files, as they tend to be the predominant type of publicly available demo files. Server-recorded demo files are often released by tournaments and competition organizers on game community sites. Additionally, players can access a service called \textit{GOTV} in-game, which broadcasts real-time games through streaming demo files as they are written by the server.

Since the demo files are effectively unstructured log files, it is important to impose a data structure on them to better facilitate data analysis. To do so, we use a demo file parser that can translate demo files into an interpretable JSON format. The parser parses the game into a series of consecutive \textit{game states}. Let $G_{r}^t$ be a game state in round $r$ at time $t$. Each game state contains the complete set of information of the world at time $t$. Thus, a game state contains data such as player locations, health, armor and grenade positions. 

\subsection{Tokenizing Game States}

Estimating situational similarity is important for a variety of sports use cases. For example, a coach may want to search for video clips in a repository containing thousands of sports plays or a player may want to tabulate their own statistics given a distinct game context. In each case, it is important that queries not only return accurate results, but also do so in a timely manner. Accurate results are especially important in a field like sports analytics, where many users, like coaches and players, may be new to working with data or model outputs, and have little experience understanding faulty output. Speed is important as we seek to improve upon the slow game review and play retrieval process. Since player locations are a large component of a game scenario, a retrieval method which can efficiently represent player locations is crucial to powering visual analytics systems which query game scenarios.

Hashing, central to many existing play clustering methods, can be used to provide quick lookup for similar scenarios. If a state can be assigned to a cluster quickly, the search space can be markedly reduced. In other sports, plays and game states may be clustered by applying clustering algorithms, such as k-means (used in Chalkboarding~\cite{sha2016chalkboarding}), on ball movement. However, as CSGO, along with most other esports, is not a ball-based sport, such techniques, like those in Chalkboarding, cannot carry over. Furthermore, clusters can greatly be affected by the choice of parameters for the clustering algorithm, and may not be interpretable. To solve the problem of quickly generating interpretable game state representations, we turn to computer-controlled \textit{bot} movement in video games.

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{imgs/nav_mesh.pdf} % map_places.png
    \Description[Navigation meshes]{Navigation meshes are graphs that represent traversable surfaces in a 3D world.}
    \caption{Navigation meshes can be constructed as graphs. ``Areas'' are traversable surfaces (nodes), and a collection of areas forms a ``Place'' (set of nodes). Typically places are collections of nodes that are close to each other. Above, we visualize areas and places for popular CSGO map Inferno.}
    \label{fig:map_places}
\end{figure}

A bot is an computer-controlled player which can play against real players, and CSGO provides the functionality for players to play against bots. To move around the virtual world, bots use a \textit{navigation mesh}, $\mathcal{N}$, which provides information on all traversable surfaces of the virtual world~\cite{snook2000simplified, navigation}. Formally, a navigation mesh for map $m$ can be thought of as a graph where $\mathcal{N}_m = (A, C)$. $A$ is a collection of \textit{areas} (nodes), and $C$ is the set of connections between areas (edges). $A$ represents the set of traversable surfaces on a given map. Each area also belongs to a set of areas which is given a human-interpretable \textit{place} identifier. Each place has a name corresponding to a predefined region on the map, like ``Bombsite A'' or ``CT Spawn''. Thus, $\forall a_i \in A, \exists P_k \textrm{ such that } a_i \in P_k$, where $k$ denotes the index of a human-interpretable place name. We show examples of areas and places extracted from navigation meshes for a few CSGO maps in Figure~\ref{fig:map_places}. The discretization of a playing space that a navigation mesh provides is not only found in video games, but also conventional sports as well. For example, some data providers discretize a playing field into zones to tabulate player fielding statistics. In soccer, it is common for coaches to discretize the pitch into different ``channels'' when talking about passing and formations. 

% https://www.baseballprospectus.com/news/article/22295/baseball-therapy-the-corner-outfield-inefficiency/

\begin{figure}
    \centering
    \includegraphics[scale=0.69]{imgs/tokenization_algorithm.pdf}
    \Description[ggViz game state tokenization]{Our game state tokenization method counts the total number of players for each discrete navigation place for each side.}
    \caption{Our tokenization process for a game state on the \textit{Inferno} map. Each colored area on the map represents a distinct place. Orange represents the Terrorist side and blue represents the Counter-Terrorists. Place names are annotated under their position in the token string. Player counts are tabulated per side on each place and concatenate into a string.}
    \label{fig:play_tokenization}
\end{figure}

To facilitate quick retrieval, we draw from previous play clustering research, which utilizes hashing of similar plays, as well as from CSGO spatial data characteristics, particularly the navigation mesh described above. Our retrieval process starts with curating a large set of CSGO game states, which we call $\mathcal{S}$. Each game state $s$ includes player positions in the form of a set of $(x, y, z)$ coordinates. From the set of player coordinates, we can determine where each player is located in $\mathcal{N}$. For each state, we assign a token, using function $T(s)$. The generated token is simply a count of the number of players of each side in each place. The token is represented as a string of the form ``$P_1 \textrm{ } P_2 \textrm{ } P_3 \textrm{ } ...$'', where $P_k$ indicates the total player count in the nodes of $P_k$. We show an example of the token creation process in Figure~\ref{fig:play_tokenization}. We calculate a token for the T and CT sides. To create a single token for the overall state, we simply concatenate the two sides' tokens. Each token is indexed in a database for fast lookup. We can also save each individual place's player count, $P_k$, separately to allow for queries on portions of a token, such as queries where a user may want to find $X$ players in place $Y$.

Considering navigation mesh $\mathcal{N}$, game state set $\mathcal{S}$ and query (game state of interest) $q$, our retrieval method $R$ returns

\begin{equation}
    R(\mathcal{N}, \mathcal{S}, q) = \{s_1, s_2, ..., s_n\}
\end{equation}

\noindent where $T(q) = T(s_i), \forall i \in \{1, 2, ..., n\}$ and $T$ is our tokenization function. To query a large set of CSGO game states, a user can provide a list of player coordinates for both the Terrorists and Counter-Terrorists, which defines $q$. Providing these player coordinates can be accomplished via a visual interface where users can draw game states of interest, like in Chalkboarding~\cite{sha2016chalkboarding}. Then, we generate the token for $q$ by calculating $T(q)$. Using this token, our retrieval system queries a database containing the set of states $\mathcal{S}$. The number of candidate states can be further reduced by imposing non-spatial constraints, such as those on equipment value, number of grenades or specific teams. One can also construct other metrics to calculate intra-token similarity and rank returned game states. For example, one could find the distance to the closest player of the same side in $s_2$ for each player in $s_1$, given two game states $s_1$ and $s_2$. Then, the total distance between $s_1$ and $s_2$ can be the sum of these distances. This method clearly becomes intractable for queries which return large sets, or for searching over the entire database of game states, but it may be suitable for smaller sets of game states. To calculate inter-token similarity, for situations where the states where the generated query token may not exist, we can consider a modified Hamming distance, where the distance between two positions in a string is the absolute value difference between them. 

We present our game state retrieval framework in Figure~\ref{fig:retrieval_system}. Our approach has the following advantages: (1) representation of spatial player information is easily interpretable as it is directly tied to human-interpretable locations, (2) limited data to store beyond three tokens for each game state and (3) performance easily scales to millions of game states. Furthermore, our method is not beholden to using navigation meshes to discretize a playing surface. As our method only relies on \textit{some} discretization of a playing surface, our method is also sport-agnostic, and can easily be adopted by other esports and conventional sports. One important distinction with previous work on play retrieval is that prior systems focused mostly on trajectory similarity. As we see in Section~\ref{sec:system}, users in esports are often searching for specific \textit{scenarios} (game states), rather than trajectories (sequences of game states). 

\begin{figure}
    \centering
    \includegraphics[scale=0.57]{imgs/token_pipeline_lato.pdf}
    \Description[ggViz game state retrieval]{Game states are preprocessed by calculating their associated token. Then, Map-Token combinations are stored in a database.}
    \caption{Our retrieval system consists of a preprocessing and retrieval step. In the preprocessing step, game states are assigned a token based on coarse player locations. This token is stored as an indexed field in a database to facilitate quick lookup. To query similar game states, a sketch containing player coordinates are translated into a token representing player locations, and then the system searches the database for game states with the same token. Candidate game states are then ranked and displayed to the user.}
    \label{fig:retrieval_system}
\end{figure}

==> 05_system_old.tex <==
\section{ggViz} \label{sec:system}
\subsection{Domain Requirements} \label{sec:domain-req}
To guide the development of our visual analytics system, we conduct interviews with primary esports stakeholders, including coaches, analysts and managers from professional CSGO teams. A1 and A2 are analysts, C1 is a coach and M1 is a manager. Each participant is employed by a professional esports organization, and has at least three years of experience in esports (median of five years). At the time of writing, A1, A2 and M1 were part of top 10 ranked teams, and C1 was part of a top 50 ranked team. We asked each expert about how they review game replays, what tasks they try to achieve and, what pain points they have in their workflow.

The stakeholders unanimously expressed that they watch and review game replays specifically for match preparation. A1 said that his organization's coach, analyst and in-game leader (the player who directs other players over the course of a match), typically prepare for matches by reviewing recent demo files of their opponents on the maps which they are most likely to play. This general workflow was also corroborated by the other professional esports stakeholders. Specifically, A1 said he looks for setups of a team under different parameters, such as how teams defend given specific equipment values or with different grenade loadouts. C1 said that their team's workflow revolved around summarizing setup tendencies of opponents under different circumstances. For example, answering a question like ``given that a team does not have much money, how do they defend a bombsite?'' is especially important. 

A1 and M1 used the CSGO in-game replay viewer to review demo files. Additionally, all interviewees also used industry-standard demo file viewers, but each agreed that there was still much work to make these viewers complete. These demo reviewers have intuitive interfaces to navigate demo files, but lack any retrieval functionality, meaning users still have to watch demo files manually to find scenarios they want. While these third-party tools are easier to use than the in-game viewer, they are often not as visually similar to the actual game. In fact, A2 said that his team eschewed the in-game viewer in favor of third-party tools and plugins. However, lack of play retrieval is still a problem in third-party tools. Because of this, each stakeholder remarked that reviewing demos can be an arduous and slow process, which prohibits any sort of large scale analysis. No stakeholder had a defined or algorithmic process to find similar plays or setups, and relied on either memory or manual search. 

%To this end, it is clear that the system will need to allow for filtering based on teams involved and on round characteristics, such as the buy types (how much money each team used) or utility level (how made grenades each team has). 
Specifically, A1, like A2, mentioned that the hardest part of the scouting process was going through demo files and finding specific instances to clip or screenshot as demonstration to players and coaches. Furthermore, A1 mentioned that he seeks to find specific game scenarios ``all the time'', and that a tool to do so would be incredibly beneficial to his workload. Specifically, A2 said that sharing points of a match can be difficult when using demo file viewers, and that 2D reconstructions were sometimes easier to share. M1 said that the ``tools aren't there to find specific spatial setups'', and for that reason, demo analysis can become quite broad and be overloading for both analysts and players. C1 said that the hardest part of scouting and game review was ``finding certain situations that are relevant to you, as you do not have the time to look through ten demo files to find enough examples''. 

From these responses, a system which can return accurate spatial setups in a fast manner could greatly improve these esports professionals' workloads. Furthermore, existing sports play retrieval systems revolved around retrieving \textit{trajectories}, and A1, C1 and M1 each added that they were instead seeking to search for particular defensive (CT) or offensive (T) positions rather than movement patterns. This is because teams often think about CSGO in terms of attacking and defending bombsites, and teams defend bombsites without much player movement.

% Query
% Support flexible queries, scalability
% Visualize round information - sheer amount of rounds means need to go thru many quickly. win probability can identify interesting rounds
% Playback functionality
% Spatial summarization

From these interviews, we develop the following requirements:

\begin{enumerate}[start=1,label={\bfseries R\arabic*}]
\item \label{req:query_context} \textit{Query game scenarios by context.} In the CSGO game review process, a user primarily watches matches with the goal of discovering \textit{strategies} that occur under specific \textit{conditions}. One of the strategies users are most interested in is understanding how teams defend bombsites. In general, strategies are represented spatially through player locations. Concerning game conditions, users want to query for strategies in specific equipment level environments, such as when teams have good equipment or bad equipment. Furthermore, most game review is done with a specific opponent in mind, meaning our system must allow a user to query matches of a particular team. The proposed design must also allow a user to query by player location and game conditions.

\item \label{req:result_metadata} \textit{Visualize game state metadata.} The game scenario search space is large, since a single CSGO game can be a few hours, and teams can play multiple times a week. One map has at minimum 16 rounds, and teams often play three maps a match, meaning matches can last multiple hours. Accordingly, users want to identify especially interesting scenarios without having to watch each scenario from the result set. Thus, the proposed design should not only return results quickly, but also allow a user to easily identify interesting game scenarios returned by the query system. Wallner~et~al. stresses the importance of visualizing high-level knowledge in post-game scenarios~\cite{DBLP:conf/chi/WallnerWBK21}.

\item \label{req:playback} \textit{Playback for player trajectories and events.} Watching a demo file is important as doing so helps users gain the full context of a state in a given round. The proposed design should provide the ability for users to playback the round in 2D, since manually watching a game is a ubiquitous activity for our stakeholders. Additionally, player actions, like grenades and kills, should also be visualized in the playback, since they influence a situation's context. Spatial characteristics were the most sought after data to visualize in post-game scenarios~\cite{DBLP:conf/chi/WallnerWBK21}.

\item \label{req:heatmap} \textit{Summarize query results.} Stakeholders are interested in summarizing tendencies of teams for presentation to other stakeholders, but especially players. For example, C1 often displayed visuals and statistics to his players before games to identify the tendencies of the opposition. The system should be able to provide an intuitive visual summary that describes a team's strategy in a given context.
\end{enumerate}

% Query interface by player position and round context
% Support flexible queries, scalability
% Visualize round information
% Playback functionality
% Spatial summarization

\subsection{System Design}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{imgs/ggviz_system_large.pdf}
    \caption{ggViz system querying a game scenario. Users can query for game scenarios in the query view (A) by sketching player positions (A1) and applying team or round filters (A2). After querying, the result view (B) shows a list of similar game scenarios. Users can navigate by looking at icons for how the round ended, or by observing win probability charts (B1). Users can also summarize the result set by viewing heatmaps of common CT/T positions for scenarios in the result set (C). Finally, users can play back the rounds that the returned game scenarios occur in through the playback view (D). The playback view shows both player trajectories (D1) and important round metadata, such as grenade usage, kills and win probability (D2).}
    \label{fig:ggviz_system}
\end{figure*}

To fulfill the requirements identified by interviews with esports experts, we developed the ggViz system, coined after the popular gaming phrase ``good game (gg)''. In Figure~\ref{fig:ggviz_system}, we see ggViz and its constituent components. ggViz contains three components, (1) the \textit{query view}, to design a query across strategies and contexts, (2) the \textit{result view}, to observe the query result set and each element's associated metadata, and (3) the \textit{playback view}, to replay the round in which the game scenario occurred and identify key points of the round.

\subsubsection{Query View}
In \boxed{\textbf{A}} we see the query view, where a user can design a query consisting of player locations and game context to find similar game scenarios (\ref{req:query_context}). Drawing from previous sports retrieval systems, we utilize a drawing interface, whereby a user can mark player positions by clicking on a map. The user differentiates between T and CT sided players through sliders to indicate side. Additionally, a user can issue two kinds of spatial queries: (1) a full query, where every player is drawn or (2) a partial query, where only a subset of players are drawn. The full query is useful for situations where users want to identify how often a team utilizes certain global strategies, which is similar to the idea of scouting a team's ``formation'' in soccer. The partial query is useful for situations when a user wants to analyze a partial region of the map, such as a bombsite. A user can mark if they want to perform a full or partial query through a slider. Once a player is placed on the map, the user can manipulate the placed player's position, which facilitates easy editing of game states. Such functionality also allows for rapid turnaround when a user tries to answer ``what if'' questions, such as what happens when a player assumes a different position on the map.

Below the spatial query view, a user can select from a variety of filters. These filters were motivated by conversations our expert users, who oftentimes found themselves searching and filtering data often on specific teams, equipment values and number of grenades on each team. In order to facilitate any targeted analysis, the team filter is particularly important, as we gathered from our experts that most game analysis is spent with a particular opposition in mind. Furthermore, much of the analysis process is also spent understanding how teams operate under specific \textit{buy types}. Buy types are determined by the aggregate equipment values of a team. For example, if a team is saving money for a round and lacks the best equipment, they are described as being in an ``eco'' or ``semi buy'' situation. Alternatively, if a team starts the rounds with the best equipment, they are said to be in a ``full buy'' situation.

% The map in the query view has its own square coordinate system, however, the CSGO has its own coordinate system which is used to determine in what area and place a player is located. Once a user clicks the submit button, the drawn game state is transformed into its corresponding in-game game coordinates. After the coordinates have been transformed, the list of players is sent as a JSON object to an API endpoint which returns the sent query's corresponding token. This token is then paired with the selected map and sent to an endpoint which returns a list of game states with the same token. End-to-end, most common queries take only around one to two seconds to return results on a database containing 100 GB of CSGO data. 

\subsubsection{Result View}
After a query is designed and executed from the query view, ggViz returns the set of results in \boxed{\textbf{B}}, the result view. Each element in the query's result set is displayed as a card which contains relevant information on that game scenario \ref{req:result_metadata}, such as the match date, competition name, round score and buy types, and how the round ended.

As the result set can be large for certain queries, users need a way to navigate through the result set to find interesting rounds. One approach to identify rounds with interesting moments is through analyzing \textit{win probability}. Win probability is a number which is an estimate for a side's chance of winning a given round. Effectively, we are estimating $P(Y_r = 1 | G_{r,t})$, where $Y_r$ is the outcome of round $r$ (1 if the CT side wins, 0 otherwise), and $G_{r,t}$ is the state of the game in round $r$ at time $t$. In order to estimate this probability, we can learn some function $f(G_{r,t}) = \widehat{Y}_{r}$, where $\widehat{Y}_{r,t}$ is the estimated outcome of round $r$ at time $t$. To learn $f$, we use the methodology in \cite{XenopoulosWPACSGO} to train an XGBoost model which predicts a side's win probability at time $t$ given $G_{r,t}$.

In each result view card, we plot the win probability of the round in which the game scenario occurred. We use a line chart which displays the win probability in the round where the game scenario occurred. CT win probability is blue, and T win probability is orange. We indicate where in the round the game scenario happened through a small circle at the top of the line chart. Finally, we also indicate important events in the round, such as when a bomb plant happened (black circle), which indicates frames that are ``pre-plant'' or ``post-plant'', since teams care about identifying ``post-plant'' situations. Essentially, the win probability chart presents a high-level overview of the round in which the game state occured. Wallner~et~al. find that players are not only interested in low-level data, but also visualizations which represent high-level concepts~\cite{DBLP:conf/chi/WallnerWBK21}.

%fix this one too
After the result view populates, there is an option to summarize the result set through a heatmap, which a user can select in the upper left corner of ggViz. To construct the heatmap, we calculate the density of one side's player locations in all game scenarios in the result set. Users can select whether they want to view the CT or the T position heatmap. By viewing the heatmap, users can identify common spots in which teams position themselves (\ref{req:heatmap}). Furthermore, by adjusting the filters in the query view, users can create different visualizations as content for other downstream stakeholders, such as players receiving a pre-game presentation from a coach.

% The aforementioned list of returned similar game states populates the game state view, shown in \boxed{\textbf{B}}. As the list of similar states can be large, we paginate the results. Each game state has relevant game state information, such as the teams involved, the game score in that state, equipment value recorded as a categorical variable and information on how the round ended. Each item has its attributes display in a scrollable list, and users can mark a state if they find it interesting. This feature is useful for users that want to reference particular game states later.

\subsubsection{Playback View}
When a user selects a game scenario of interest, the playback view in \boxed{\textbf{C}} populates. The playback view allows a user to view the round in which the game scenario occurred (\ref{req:playback}). Player positions are displayed on the map. Below the map is a slider which one can use to animate the round frame by frame. This feature acts as a quick substitute for video review, which typically takes place by playing back a demo file. Playing a demo file incurs a lengthy setup cost, as doing so typically requires running CSGO and loading a demo file. This greatly prohibits one from quickly switching between rounds in different demo files. However, if a user wants to view the demo file, we display a button to the right of the playback slider which will launch the CSGO game to watch the demo file.

% In ggViz, if a user wants to view the demo to view the selected game state and round more in depth, they only need to select the card in the result view, which will retrieve the trajectories for that specific round. 

By presenting the whole round for playback, a user can accomplish a variety of tasks. For example, a user can look at the game scenarios prior to selected one to develop a sense for how the selected game scenario came to be. On the other hand, a user can view the part of the round which occurs after the selected state to uncover what was the result of a particular scenario. Below the slider are tabs to view the round win probability, kills and grenades. In the win probability graph, we show added context for the round the user is reviewing. As major round events, like kills, are highly correlated with win probability~\cite{XenopoulosWPACSGO}, a user is quickly able to visit important round events. In the ``kill'' and ``grenades'' tab, a user can click to go to the frame where the kill occurred or grenade was thrown. These specific player events add more context to the 2D view, and can help a user understand the circumstances of a given round.

\subsection{Implementation}
Early play retrieval systems, such as Chalkboarding, relied on non-web based interfaces. However, web-based applications are now ubiquitous, are able to support data-intensive workloads, such as play retrieval, and are easy to access for a wide array of users. As such, we prioritized ggViz to be accessible via a web-based client. ggViz is implemented with a client-server architecture. The client is a web application built with Angular, which renders the spatial query, result and round playback views. Using Flask, we develop an API which fulfills client requests, and in particular implements the retrieval system described in Figure~\ref{fig:retrieval_system}. The API interacts with a SQL database that contains roughly 100 GB of data on 1,600 professional matches occurring from April 1st, 2020 to August 31st, 2020. This corresponds to over 10 million game states and over 100 million player locations. Game states are stored in a clustered SQL index, where the index is created on $(Map, Token)$ combinations. We acquired the demo files from the popular Counter-Strike website HLTV.org. We parsed each demo file using the \texttt{awpy} CSGO demo parser at a frequency of one state per second~\cite{XenopoulosWPACSGO}. 

Both the client and server architectures are modular. The visual components, such as the playback view or query interface, can easily be extended to other systems. This is important for future systems, as most web-based visual analytics applications in esports will ostensibly require some 2D playback or map-based view. Additionally, our API can broadly support many CSGO specific applications, and can easily be extended by teams, organizations and players. For example, our API contains endpoints to retrieve event data, such as grenades, kills and damages, or player-tracking data. These endpoints can be used to retrieve data to power machine learning models or other visual analytics systems. Generally, these endpoints and data can also be used for 2D CSGO round playback.

==> 06_evaluation_old.tex <==
\section{Evaluation} \label{sec:evaluation}
To evaluate the usefulness of ggViz for esports analytics, we conduct think-aloud expert interviews, where we showcased ggViz to staff from professional esports teams and recorded their feedback. Additionally, we showcase two use cases of ggViz, which were identified as routine game analysis tasks by CSGO experts.

\subsection{Expert Interviews}
To evaluate ggViz, we held ``think aloud'' interviews with the four esports experts mentioned in the pre-design interviews in section~\ref{sec:domain-req}, as well as an additional analyst, denoted A3. A3 was part of the same esports organization as C1. Although we only used five experts, four of the five experts were working for, at the time, Top 10 ranked teams. The experts were free to use ggViz in whichever way they wanted. While doing so, the experts were encouraged to speak about their thought process. During each interview, which lasted an hour, we recorded the expert's thoughts on the system, as well as noted how each expert used ggViz.  
\subsubsection{Filtering Scenarios}
Each expert's first actions with ggViz were to confirm tendencies for their own team. However, before drawing scenarios of interest, each user first inspected and applied the filters below the map query view. Of particular note were the team, round equipment and grenade count filters. Almost all queries that the users issued used these filters, which is consistent with the conclusions from the pre-design interviews. Before each query, each expert would vocalize what situation they wanted to find. In every instance, each expert referenced the ``buy type'' of a particular side, which is a rough hierarchy of equipment values. For example, an ``eco'' round is one where a team spends little to no money for a round in an effort to save money, and a ``full buy'' is one where a team acquires the best guns available. Our filters used the same nomenclature, which the experts appreciated. Overall, A2 remarked that the filtering was quite extensive and was satisfied that the filters corresponded to his team's general analysis workflows, saying ``the filters are exactly what we need''.

\subsubsection{Drawing Game Scenarios}
After selecting the filters, each expert would then draw the game state, which normally took under 10 seconds. All participants found the interface intuitive as the map view was familiar to anybody who has played the game. A1 mentioned that such an interface is ``super useful for coaches and for match preparation''. While ggViz allows a user to specify both CT and T players, most expert queries issued either partial queries, or full queries on a specific side. M1 and C1 said that he especially appreciated the ability to perform single-sided and partial queries, as a large part of their workflows are seeing how specific teams spatially distribute themselves on the CT side, irrespective of how the T side is distributed. After later explaining the retrieval process to the experts, each user's drawing speed was much faster, since each expert understood that their game state drawings need not be exact, and they spent less time on getting players in exact locations. We also observed A1 and A2 try to understand the retrieval methodology further by placing players near the borders of navigation mesh surfaces and seeing how the result set changed. 

\subsubsection{Viewing Retrieval Results}
% review
The retrieved game states, along with the speed of the retrieval, were well received. M1 said that the similar plays looked ``great, they correspond to what I'm looking for''. Additionally, M1 mentioned that the query speed was well-suited to delivering fast turnaround for his workload. A2 remarked that the retrieval was ``fluid and fast, I don't have to wait forever to find what I want'' and that the retrieved game states made sense given all of his queries. C1 said ``I drew the exact setups I know my team uses, and I can see all of them within seconds. The returned states are excellent''. A3 remarked that the system is ``very accurate and returns the game states I expect, and at the point in the round I expect them to occur''. The amount of time the experts spent analyzing the result set was variable. For example, C1 would quickly look at a few rounds (two to four), since his workflow was trying to understand how a team's CT sets up. C1 found the heatmap feature useful as well, since he could use these heatmaps to send to players. Conversely, A1 would spend a few minutes on a single game scenario by playing back the round's trajectories multiple times and jumping to different points in the round in order to understand the specific events of that round. Experts found that the win probability graph was useful in finding important points in a round as it clearly identified kills and deaths through large increases or decreases in win probability.

\subsubsection{Exploring Tactics On a Large Scale}
While team filters were present on almost all queries, A2 started to use the tool without a team filter towards the end of his interview. He then suggested that although ggViz's direct use case is for game review, ggViz could also be used for a large scale analysis since the database of games was large and the retrieval speed was fast. A2 mentioned that most coaches and analysts in the CSGO community watch demos from their own team or their upcoming opposition, and thus lack the time to watch game replays in-depth from other top teams, but ggViz could allow them to learn more from other teams in a faster manner than going through individual demo files.

\subsubsection{Expert Feedback}
The feedback from the participants was very positive and each of them were excited to use the tool in depth and to suggest new features for future work. A2 said that the system solved his problem of finding specific game setups and contexts. C1 stated that he saw potential for ggViz to be ``more valuable than the other tools out there''. A2, C1 and M1 expressed interest that future versions of ggViz include more analytics, such as assigning values to player actions. One option is to assign values using the change in win probability, as is done in~\cite{XenopoulosWPACSGO} The majority of the negative feedback of ggViz relied mostly on cosmetic details in the round playback view, such as what directions players were viewing or animations for grenades. One limitation of ggViz is dealing with height. Some maps in CSGO have buildings with multiple floors. In situations like these, a single 2D view may be confusing. To address this, we can use multiple maps to display locations, where each map visualize a certain height level. For example, in CSGO there already exists ``upper'' and ``lower'' images for Nuke and Vertigo, two maps with large height differences. 

\subsection{Use Case: Analyzing Retakes}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{imgs/retakes_ggviz.pdf}
    \caption{S1, S2 and S3 detail three possible retake strategies for the Counter-Terrorists in a 2 CT versus 3 T scenario for the B bombsite on the \textit{Inferno} map. As shown in Table~\ref{tab:retake-wins}, retakes originating from ``Banana'' have a lower success rate than those from ``CT''. The banana and CT areas are labeled in S1.}
    \label{fig:retake-examples}
\end{figure}

Understanding how a given game state affects the subsequent game state is an important part of match analysis. C1 said that the use case he found ggViz most useful was for analyzing specific CT defensive setups and retake scenarios. A \textit{retake} is a common maneuver in CSGO, whereby the CT sided team attempts to regain control of a bombsite where the T team has planted the bomb. In fact, A1 also mentioned that understanding a team's retake strategy is key game preparation point. ggViz is uniquely positioned to analyze retakes, and how teams play them, as one can not only identify retake strategies but also retake defense setups. A user can define a given bombsite defense from the T side, and then analyze the retake strategies on similar defense setups. Even though there is no definitive ``retake'' filter in ggViz, simply placing T players in common retake defense places, and enforcing a bomb exploded or defused filter, ensures that the returned states are mostly retakes.

Let's consider a case where a user is interested in retake strategies for a two CT versus three T situation for bombsite B on the map \textit{de\_inferno}. We will assume that all three T players are defending from inside bombsite B, which is a common strategy verified by our experts. A two CT on three T situation is not uncommon, as usually two to three CTs defend a bombsite, so if a T side gains control of a bombsite, it is likely the other CT players were killed in the process. To isolate retake scenarios, we can filter for rounds that ended with the bomb exploding, the CT side being killed or the bomb being defused. In the former two scenarios, the T side wins the round. For the latter scenario, the CT side wins the round. By analyzing successful and unsuccessful retakes, we can parse through example rounds to find successful strategies. In our example, there are two general paths a player can take to retake the B bombsite: the ``banana'' or the ``CT'' path. In Figure~\ref{fig:retake-examples} we show three queried game situations. Because the B bombsite is considered a single place in the navigation mesh, we just place the three T players in the bombsite. In S1, there are two players in the CT path. In S2, there are two players in the banana path. In S3, there is one player in the CT and one player in the banana path.

When a user issues these queries, they can quickly parse through the returned game states and see the outcomes by viewing the round end icons, which are colored by the winning side and represent how the round ended, such as through a bomb explosion, defuse, and so on. We present the summarized round end results for each situation query in Table~\ref{tab:retake-wins}. Although a two CT versus three T retake is already a difficult situation for the CT side to win, it is clear that coming from the banana direction is the least advantageous, and rarely results in a win for the CT side. Additionally, we see that S1 is the most common situation in our database of CSGO games, indicating the community typically uses the highest win rate retake strategy.

\begin{table}[]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Situation} & \textbf{T Wins} & \textbf{CT Wins} & \textbf{CT Win Rate} \\ \midrule
S1 & 51 & 6 & 12\% \\
S2 & 19 & 1 & 5\% \\
S3 & 7 & 0 & 0\% \\ \bottomrule
\end{tabular}%
\caption{Situations which involve attacks emanating from the banana area (S2 and S3) have a lower win rate than those from the CT area (S1).}
\label{tab:retake-wins}
\end{table}

\subsection{Use Case: Summarizing Team Setups}
In the previous use case, we demonstrated the use of ggViz for understanding the events that occur \textit{after} a given game state. To do so, one must primarily use the result view and playback view. However, it is also important to summarize the result set itself. For example, a coach may want to create a visualization to share among players that describes how an opposing team defends a specific bombsite.

Consider the query in Figure~\ref{fig:heatmap}. Here, we issue a partial query that places two players on B bombsite in the map Inferno. Typically, two players defend the B bombsite on the CT side. We are interested in summarizing what positions these two players are likely to play. Furthermore, we are also interested how these positions differ under different buy conditions, such as a full buy or a semi-buy. This is a common task performed by coaches and analysts to find what they call a team's ``default''. 

In Figure~\ref{fig:heatmap}, we see the player position heatmaps for scenarios with two players on bombsite B under different buy scenarios. We provide the callouts for reference in the right side of the figure. We can see that there are clear positioning distinctions between the different buy types. For example, in full buys, players are more likely to position themselves at 1st/2nd and Dark. In semi buys, we see that players are likely to play closer to banana, and leaving Dark and 1st/2nd sparsely occupied. Interestingly, we see that in pistol rounds, players take positions deep in the bombsite, such as at Coffins or New Box.

\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{imgs/heatmaps.pdf}
    \caption{We issue a partial query for two CT players on Inferno's B bombsite. We generate heatmaps for four different buy scenarios, and we provide the callouts for reference. We see that in full buy scenarios, the CT players are more likely to position themselves at 1st/2nd and Dark. In Semi Buys, players are more likely to position themselves closer to Banana. }
    \label{fig:heatmap}
\end{figure}


%\subsection{Understanding Map Control}

%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{imgs/map_control_example.pdf}
%    \caption{We query a scenario in \boxed{\textbf{A}} where the T side has split their offensive. This scenario is quite rare and indicates that the T's have obtained substantial map control. In \boxed{\textbf{B}} we see that the T side is clustered in the middle of the map. In \boxed{\textbf{C}}, the two T's in the upper part of the map use grenades, which usually indicates that the team is pushing. However, in \boxed{\textbf{D}}, we see that the two players on the left have maintained their position, while the players on the right are wrapping around and throwing a smoke grenade to mask their movement.}
%    \label{fig:map-control}
%\end{figure*}

%In the previous case, we demonstrated the use of ggViz for understanding the events that occur \textit{after} a given game state. However, it is almost important in match analysis to understand the \textit{why} of a current game state. Accordingly, ggViz can be used to understand how preceding game states affect the current one. In their interviews, each expert mentioned the phrase ``map control''. Map control is the process by which the two teams vie for dominance over spatial regions of the map. C1 and M1 said that playback functionality would be useful for understanding map control. A1 regarded understanding map control strategies as one of the most arduous aspects of scouting opponents. Below, we analyze map control on \textit{de\_inferno}. 

%Consider the query made in the top image in Figure~\ref{fig:map-control}. This distribution of T players, as indicated from talking to our CSGO experts, indicates that the T side has obtained control over large parts of the map, particularly the middle, which is regarded as important. The specific setup of three T players in the middle is a strong formation as it allows for the T side to attack either the bombsite (shaded red box) in the top left or the bottom right of the map. By observing what happened before similar states, we can observe how the T side obtained such map control. Figure~\ref{fig:map-control} shows the game states before and after a candidate state state.

%In the above example, we also see how the use of grenades is important to gaining and maintaining map control. In
%\boxed{\textbf{C}}, the two T sided players throw their grenades at the B bombsite, which typically indicates a team is making an attempt to gain control of that bombsite. This maneuver allows the other three T players to wrap around from the middle of the map. In \boxed{\textbf{D}}, these three T players throw a smoke grenade to mask their movement and prevent the other team from pushing their position. Using ggViz, we can understand how the T sided team moved and used grenades as a team to gain such an advantageous position.

